Theoretical Analysis of Offline Imitation With Supplementary Dataset

Behavioral cloning (BC) can recover a good policy from abundant expert data, but may fail when expert data is insufficient. This paper considers a situation where, besides the small amount of expert data, a supplementary dataset is available, which can be collected cheaply from sub-optimal policies. Imitation learning with a supplementary dataset is an emergent practical framework, but its theoretical foundation remains under-developed. To advance understanding, we first investigate a direct extension of BC, called NBCU, that learns from the union of all available data. Our analysis shows that, although NBCU suffers an imitation gap that is larger than BC in the worst case, there exist special cases where NBCU performs better than or equally well as BC. This discovery implies that noisy data can also be helpful if utilized elaborately. Therefore, we further introduce a discriminator-based importance sampling technique to re-weight the supplementary data, proposing the WBCU method. With our newly developed landscape-based analysis, we prove that WBCU can outperform BC in mild conditions. Empirical studies show that WBCU simultaneously achieves the best performance on two challenging tasks where prior state-of-the-art methods fail.

==> bc_gfa.tex <==
\section{Behavioral Cloning with General Function Approximation}
\label{sec:bc_gfa}


In the main text, the theoretical analysis for BC-based algorithms considers the tabular setting in policy learning where a table function represents the policy. Here we provide an analysis of BC with \emph{general function approximation} in policy learning. Notice that the algorithms considered in this paper (i.e., BC, NBCU and WBCU) can be unified under the framework of maximum likelihood estimation (MLE)\footnote{Among these algorithms, the main difference is the weight function in the MLE objective; see Equations \eqref{eq:bc_opt}, \eqref{eq:bc_union} and \eqref{eq:dwbc}.}. Therefore, the theoretical results in the main text can also be extended to the setting of general function approximation by a similar analysis. 



We consider BC with general function approximation, which is the foundation of analyzing NBCU and WBCU. In particular, we assume access to a policy class $\Pi = \{ \pi = (\pi_1, \pi_2, \ldots, \pi_h): \; \pi_h \in \Pi_h, \; \forall h \in [H]  \}$ and $\Pi_h = \{ \pi_h : \gS \rightarrow \Delta (\gA) \}$, where $\pi_h$ could be any function (e.g., neural networks). For simplicity of analysis, we assume that $\Pi$ is a finite policy class. The objective of BC is still 
\begin{align*}
  \pi^{\bc} \in  \max_{\pi \in \Pi} \sum_{h=1}^{H} \sum_{ (s, a) \in \gS \times \gA} \widehat{d^{\expert}_h}(s, a) \log \pi_h(a|s),
\end{align*}
but we do not have the analytic solution as in \cref{eq:pi_bc}.


\begin{thm}
\label{thm:bc_imitation_gap_gfa}
Under \cref{asmp:dataset_collection}. In the general function approximation, additionally assume that $\piE \in \Pi$, we have
\begin{align*}
    \expect \ls V (\piE) - V (\pi^{\bc}) \rs \lesssim \min \lb H, H^2\sqrt{\frac{\log (|\Pi| H N_{\expert})}{N_{\expert}}} \rb
\end{align*}
\end{thm}

Compared with \cref{thm:bc_expert}, we find that the only change in theoretical bound is that $\gO(|\gS|/N_{\expert})$ is replaced with $\gO(\sqrt{\log ( |\Pi|)/ N_{\expert}})$. We note that such a change also holds for other algorithms (e.g., NBCU and WBCU). Therefore, our theoretical implications remains unchanged.


\begin{proof}[Proof of \cref{thm:bc_imitation_gap_gfa}]
We apply the policy difference lemma in \citep{kakade2002pg} and obtain that
\begin{align*}
    V (\piE) - V (\pi^{\bc}) &= \sum_{h=1}^H \expect_{s_h \sim d^{\piE}_h (\cdot)} \ls Q^{\pi^{\bc}}_h (s_h, \piE_h (s_h)) - \sum_{a \in \gA} \pi^{\bc}_h (\cdot|s_h) Q^{\pi^{\bc}}_h (s_h, a)  \rs
    \\
    &\leq \sum_{h=1}^H \expect_{s_h \sim d^{\piE}_h (\cdot)} \ls Q^{\pi^{\bc}}_h (s_h, \piE_h (s_h)) (1-\pi^{\bc}_h (\piE_h (s_h)|s_h))  \rs  
    \\
    &\leq H \sum_{h=1}^H \expect_{s \sim d^{\piE}_h (\cdot)} \ls \expect_{a \sim \pi^{\bc}_h (\cdot|s)} \ls \indict \lb a \not= \piE_h (s) \rb \rs \rs
    \\
    &= H \sum_{h=1}^H \expect_{s_h \sim d^{\expert}_h (\cdot)} \ls \TV \lp \piE_h (\cdot|s_h), \pi^{\bc}_h (\cdot|s_h)  \rp \rs. 
\end{align*}
With Theorem 21 in \citep{agarwal2020flambe}, when $|\gDE| \geq 1$, for any $\delta \in (0, 1)$, with probability at least $1-\delta$ over the randomness within $\gDE$, we have that
\begin{align*}
    \expect_{s_h \sim d^{\expert}_h (\cdot)} \ls \TV^2 \lp \piE_h (\cdot|s_h), \pi^{\bc}_h (\cdot|s_h)  \rp \rs \leq 2 \frac{\log (|\Pi| / \delta)}{|\gDE|}.
\end{align*}
With union bound, with probability at least $1-\delta$, for all $h \in [H]$, it holds that
\begin{align*}
    \expect_{s_h \sim d^{\expert}_h (\cdot)} \ls \TV^2 \lp \piE_h (\cdot|s_h), \pi^{\bc}_h (\cdot|s_h)  \rp \rs \leq 2 \frac{\log (|\Pi| H / \delta)}{|\gDE|}, 
\end{align*}
which implies that 
\begin{align*}
     V (\piE) - V (\pi^{\bc}) &\leq  H \sum_{h=1}^H \expect_{s_h \sim d^{\expert}_h (\cdot)} \ls \TV \lp \piE_h (\cdot|s_h), \pi^{\bc}_h (\cdot|s_h)  \rp \rs
    \\
    &\overset{(a)}{\leq}  H \sum_{h=1}^H \sqrt{ \expect_{s_h \sim d^{\expert}_h (\cdot)} \ls \TV^2 \lp \piE_h (\cdot|s_h), \pi^{\bc}_h (\cdot|s_h)  \rp \rs}
    \\
    &\leq \sqrt{2} H^2 \sqrt{\frac{\log (|\Pi| H / \delta)}{|\gDE|}}.
\end{align*}
Inequality $(a)$ follows Jensen's inequality. Taking expectation over the randomness within $\gDE$ yields that
\begin{align*}
    \expect_{\gDE} \ls V (\piE) - V (\pi^{\bc}) \rs &\leq \delta H + (1-\delta)  \sqrt{2} H^2 \sqrt{\frac{\log (|\Pi| H / \delta)}{|\gDE|}}
    \\
    &\overset{(a)}{=} \frac{H}{2|\gDE|} + \lp 1-\frac{1}{2 |\gDE|} \rp \sqrt{2} H^2 \sqrt{\frac{\log (2|\Pi| H |\gDE|)}{|\gDE|}}
    \\
    &\leq \lp  \sqrt{2} + 1 \rp H^2 \sqrt{\frac{\log (2|\Pi| H |\gDE| )}{|\gDE|}}
    \\
    &\leq 4 H^2 \sqrt{\frac{\log (4|\Pi| H |\gDE| )}{|\gDE|}}. 
\end{align*}
Equation $(a)$ holds due to the choice that $\delta = 1/(2 |\gDE|)$. For $|\gDE| = 0$, we directly have that 
\begin{align*}
    \expect_{\gDE} \ls V (\piE) - V (\pi^{\bc}) \rs \leq H.
\end{align*}
Therefore, for any $|\gDE| \geq 0$, we have that
\begin{align*}
    \expect_{\gDE} \ls V (\piE) - V (\pi^{\bc}) \rs \leq 4 H^2 \sqrt{\frac{\log (4|\Pi| H \max\{ |\gDE|, 1 \} )}{\max\{ |\gDE|, 1\}}}. 
\end{align*}
We consider a real-valued function $f (x) = \log (cx) / x, \; \forall x \geq 1$, where $c = 4|\Pi| H$. Its gradient function is $f^\prime (x) = (1-\log (cx)) / x^2 \leq 0, \; \forall x \geq 1$. Then we know that $f (x)$ is decreasing as $x$ increases. Furthermore, we have that $\max\{ |\gDE|, 1\} \geq (|\gDE| + 1)/2, \; \forall |\gDE| \geq 0$. Then we obtain
\begin{align*}
    \expect_{\gDE} \ls V (\piE) - V (\pi^{\bc}) \rs &\leq 4 H^2 \sqrt{\frac{\log (4|\Pi| H \max\{ |\gDE|, 1 \} )}{\max\{ |\gDE|, 1\}}}
    \\
    &\leq 4 H^2 \sqrt{\frac{2 \log (4|\Pi| H (|\gDE|+ 1) )}{|\gDE|+ 1}}. 
\end{align*}
Taking expectation over the random variable $|\gDE| \sim \text{Bin} (N_{\tot}, \eta)$ yields that
\begin{align*}
    \expect \ls V (\piE) - V (\pi^{\bc}) \rs &\leq 4 H^2 \expect \ls \sqrt{\frac{2 \log (4|\Pi| H (|\gDE|+ 1) )}{|\gDE|+ 1}} \rs
    \\
    &\overset{(a)}{\leq} 4 H^2 \sqrt{\expect \ls \frac{2 \log (4|\Pi| H (|\gDE|+ 1) )}{|\gDE|+ 1} \rs}  .
\end{align*}
Inequality $(a)$ follows Jensen's inequality. We consider the function $g (x) = -x \log (x/c) , \; \forall x \in (0, 1]$, where $c = 4 |\Pi| H$.
\begin{align*}
    g^\prime (x) = - (\log (x/c) + 1) \geq 0, \;  g^{\prime \prime} (x) = - \frac{1}{x} \leq 0, \; \forall x \in (0, 1].
\end{align*}
Thus, $g (x)$ is a concave function. By Jensen's inequality, we have that $\expect [g(x)] \leq g (\expect [x])$. Then we can derive that
\begin{align*}
    \expect \ls V (\piE) - V (\pi^{\bc}) \rs & \leq 4 H^2 \sqrt{\expect \ls \frac{2 \log (4|\Pi| H (|\gDE|+ 1) )}{|\gDE|+ 1} \rs}
    \\
    &= 4 \sqrt{2} H^2 \sqrt{ \expect \ls g \lp \frac{1}{|\gDE| + 1} \rp \rs}
    \\
    &\leq 4 \sqrt{2} H^2 \sqrt{ g \lp \expect \ls  \frac{1}{|\gDE| + 1} \rs \rp}
    \\
    &\overset{(a)}{\leq} 4 \sqrt{2} H^2  \sqrt{ g \lp \frac{1}{N_{\expert}} \rp} 
    \\
    &\leq 4 \sqrt{2} H^2\sqrt{ \frac{ \log (4|\Pi| H N_{\expert} )}{N_{\expert}}}.
\end{align*}
In inequality $(a)$, we use the facts that $g^\prime (x) \geq 0$ and $\expect \ls  1/(|\gDE| + 1) \rs \leq 1/N_{\expert} $ from \cref{lem:binomial_distribution}. We complete the proof.
\end{proof}


==> defs.tex <==
\newcommand{\ones}{\mathbf 1}
\newcommand{\reals}{{\mathbb{R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\symm}{{\mbox{\bf S}}}  %

\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\rank}{\mathop{\bf rank}}
\newcommand{\conv}{\mathop{\bf conv}}
\newcommand{\prox}{\mathbf{prox}}


\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\Co}{{\mathop {\bf Co}}} %
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\epi}{\mathop{\bf epi}} %
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\dom}{\mathop{\bf dom}} %
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\sign}{\mathop{\bf sign}}
\newcommand{\avg}{\operatorname{avg}}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}

\newcommand{\tra}{\mathrm{tr}}

\newcommand{\grad}{\texttt{g}}
\newcommand{\myvert}{\,\vert \,}

\newcommand{\dquote}[1]{``#1''}



==> experiments.tex <==
\section{Experiments}
\label{appendix:experiments}

\subsection{Experiment Details}
\label{appendix:experiment_details}



\textbf{Dataset Collection.}  We train an online SAC agent \citep{haarnoja2018sac} with 1 million steps using the rlkit codebase\footnote{\url{https://github.com/rail-berkeley/rlkit}}, which is the same as benchmark dataset D4RL\footnote{\url{https://github.com/Farama-Foundation/D4RL}}. We use the deterministic policy as the expert policy, which is common in the literature \citep{ho2016gail} since the deterministic policy usually gives a better performance than the stochastic policy; see \cref{fig:sac} for the training curves of online SAC. 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{images/rlkit_sac.pdf}
    \caption{Training curves of online SAC.}
    \label{fig:sac}
\end{figure}



In our experiments, the expert dataset has 1 expert trajectory that is collected by the trained SAC agent. Two tasks differ in the supplementary dataset.

\textbf{Noisy Expert Task.} The supplementary dataset has 10 clean expert trajectories and 5 noisy expert trajectories. For noisy trajectories, the action labels are replaced with random actions (drawn from $[-1, 1]$). 


\textbf{Full Replay Task.} The supplementary dataset is from the replay buffer of the online SAC agent, which has 1 million samples (roughly 1000+ trajectories). 


\textbf{Algorithm Implementation.} The implementation of DemoDICE is based on the original authors' codebase\footnote{\url{https://github.com/KAIST-AILab/imitation-dice}}. Same as DWBC\footnote{\url{https://github.com/ryanxhr/DWBC}}. We have fine-tuned the hyper-parameters of DemoDICE and DWBC in our experiments but find that the default parameters given by these authors work well. Following \citep{kim2022demodice}, we normalize state observations in the dataset before training for all algorithms.


We use gradient penalty (GP) regularization in training the discriminator of WBCU. Specifically, we add the following loss to the original loss \eqref{eq:discriminator_opt}:
\begin{align*}
    \min_{\theta} \lp \lnorm g(s, a; \theta) \rnorm - 1 \rp^2,
\end{align*}
where $g$ is the gradient of the discriminator $c(s, a; \theta)$.

The implementation of NBCU and WBCU is adapted from DemoDICE's. In particular, both the discriminator and policy networks use the 2-layers MLP with 256 hidden units and ReLU activation. The batch size is 256 and  learning rate (using the Adam optimizer) is $0.0003$ for both the discriminator and policy. The number of training iterations is 1 million. We use $\delta = 0$ and GP=1, unless mentioned. Please refer to our codebase\footnote{\url{https://github.com/liziniu/ILwSD}} for details. 


All experiments are run with 5 random seeds. 






\subsection{Additional Results}


In this section, we report the exact performance of trained policies for each MuJoCo locomotion control task. Training curves are displayed in \cref{fig:noisy_expert} and \cref{fig:full_replay}.  The evaluation performance of the last 10 iterations is reported in \cref{tab:noisy_expert} and  \cref{tab:full_replay}. The normalized score on a particular environment is calculated by the following formula. 
\begin{align*}
    \text{Normalized Score} = \frac{\text{Algorithm Performance} - \text{Random Policy Performance}}{\text{Expert Policy Performance} - \text{Random Policy Performance}}.
\end{align*}
In \cref{tab:noisy_expert} and \cref{tab:full_replay}, the normalized score is averaged over 4 environments.

Training curves of WBCU and DemoDICE with gradient penalty are displayed in \cref{fig:noisy_expert_wbcu}, \cref{fig:full_replay_wbcu}, \cref{fig:noisy_expert_demo_dice}, and \cref{fig:full_replay_demo_dice}.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.45\linewidth]{images/demo_dice_gp.pdf}
    \caption{Averaged normalized scores of trained policies of DemoDICE with gradient penalty. Experiments show that the gradient penalty regularization also matters for DemoDICE.}
    \label{fig:demo_dice_gp}
\end{figure}


\begin{table}[htbp]
\centering
\caption{Performance of the trained policies by BC, DemoDICE \citep{kim2022demodice}, DWBC \citep{xu2022discriminator}, NBCU (\cref{algo:nbcu}), and WBCU (\cref{algo:wbcu}) on the noisy-expert task. Numbers correspond to the averaged evaluation return over 5 random seeds ($\pm$ indicate the standard deviation); a lager return means  better performance (same as other tables). }
\label{tab:noisy_expert}
\begin{tabular}{@{}c|llll|l@{}}
\toprule
            & Ant-v2  & HalfCheetah-v2 & Hopper-v2 & Walker2d-v2 & Normalized Score\\ \midrule
Random      &   -325.6        & -280            & -20       & 2     & 0\% \\  
Expert      &   5229          & 11115           & 3589      & 5082   & 100\%      \\ \midrule
BC &  \meanstd{1759}{287}               &  \meanstd{931}{273}            &  \meanstd{2468}{164}      & \meanstd{1738}{311}   &    38\%       \\
\midrule 
DemoDICE(GP=0)    &  \meanstd{1893}{181}               &  \meanstd{2139}{277}           &  \meanstd{1823}{169}                          &  \meanstd{563}{34}                   & 31\%            \\ 
DemoDICE(GP=1)    &  \meanstd{2492}{235}               &  \meanstd{5553}{501}           &  \meanstd{1320}{319}                          &  \meanstd{1153}{220}                   & 40\%            \\ 
DemoDICE(GP=10)    &  \meanstd{2523}{244}               &  \meanstd{6020}{346}           &  \meanstd{1990}{90}                          &  \meanstd{1685}{160}                   & 49\%            \\ 
DWBC    &    \meanstd{3270}{238}             &   \meanstd{5688}{557}                    &  \meanstd{3317}{59}                    &  \meanstd{1985}{175}                 & 62\%              \\ \midrule 
NBCU   &     \meanstd{3259}{159}          &  \meanstd{5561}{539}            &  \meanstd{558}{23}     &      \meanstd{518}{56}  & 35\%      \\
WBCU(GP=0)   &  \meanstd{738}{179}               &  \meanstd{3828}{333}            &  \meanstd{2044}{111}      & \meanstd{477}{81}          & 30\% \\
WBCU(GP=1)   &  \meanstd{2580}{224}               &  \meanstd{8274}{488}            &  \meanstd{3217}{203}      & \meanstd{1932}{329}          & 64\%  \\ 
WBCU(GP=10)   &  \meanstd{2130}{259}               &  \meanstd{7813}{472}            &  \meanstd{2930}{229}      & \meanstd{1510}{476}          & 57\%   \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[htbp]
\centering
\caption{Performance of the trained policies by BC, DemoDICE \citep{kim2022demodice}, DWBC \citep{xu2022discriminator}, NBCU (\cref{algo:nbcu}), and WBCU (\cref{algo:wbcu}) on the full-replay task. }
\label{tab:full_replay}
\begin{tabular}{@{}c|llll|l@{}}
\toprule
            & Ant-v2  & HalfCheetah-v2 & Hopper-v2 & Walker2d-v2 & Normalized Score \\ \midrule
Random      &   -325.6        & -280            & -20       & 2     & 0\%  \\  
Expert      &   5229          & 11115           & 3589      & 5082   & 100\%      \\ \midrule
BC &  \meanstd{1759}{287}               &  \meanstd{931}{273}            &  \meanstd{2468}{164}      & \meanstd{1738}{311}   &    38\%       \\
\midrule 
DemoDICE(GP=0)    &  \meanstd{4650}{216}               &  \meanstd{9882}{270}           &  \meanstd{39}{0}                          &  \meanstd{4149}{288}                 &  66\%             \\ 
DemoDICE(GP=1)    &  \meanstd{5009}{98}               &  \meanstd{10701}{70}           &  \meanstd{3427}{104}                          &  \meanstd{4560}{146}                 &  94\%             \\ 
DemoDICE(GP=10)    &  \meanstd{5000}{124}               &  \meanstd{10781}{67}           &  \meanstd{3394}{93}                          &  \meanstd{4537}{125}                 &  94\%             \\ 
DWBC    &      \meanstd{2951}{155}           &   \meanstd{1485}{377}                              &     \meanstd{2567}{88}                      &  \meanstd{1572}{225}                & 44\%               \\ \midrule 
NBCU  &   \meanstd{4932}{148} & \meanstd{10566}{86} & \meanstd{3241}{276} & \meanstd{4462}{105} & 92\%  \\
WBCU(GP=0)   &  \meanstd{483}{79}               &  \meanstd{-242}{101}            &  \meanstd{346}{93}      & \meanstd{15}{15}       & 6\% \\
WBCU(GP=1)   &  \meanstd{4935}{108}               &  \meanstd{10729}{74}            &  \meanstd{3390}{132}      & \meanstd{4509}{142}       & 94\%  \\
WBCU(GP=10)   &  \meanstd{4858}{95}               &  \meanstd{10751}{41}            &  \meanstd{3436}{37}      & \meanstd{4403}{88}       & 93\%    \\ \bottomrule
\end{tabular}
\end{table}


\begin{rem}   \label{rem:dataset_coverage}
Readers may realize that NBCU actually is better than BC on the Ant-v2 and HalfCheetah-v2 environments for the noisy-expert task, which seems to contradict our theory. We clarify there is no contradiction. In fact, our theory implies that in the worst case, NBCU is worse than BC. As we have discussed in the main text, state coverage matters for NBCU's performance. For the noisy expert task, we visualize the state coverage in \cref{fig:noisy_expert_dataset_coverage}, where we use Kernel PCA\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.decomposition.KernelPCA.html}. We use the \dquote{poly} kernel.} to project states. In particular, we see that the state coverage is relatively nice on Ant-v2 and HalfCheetah-v2, and somewhat bad on Hopper-v2 and Walker2d-v2. This can help explain the performance difference among these environments in \cref{tab:noisy_expert}.
\end{rem}

\begin{figure}[htbp]
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=0.95\linewidth]{images/ant_pca.pdf}
\caption{Ant-v2.}
\end{subfigure}
\hfill
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=0.95\linewidth]{images/halfcheetah_pca.pdf}
\caption{Halfcheetah-v2.}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=0.95\linewidth]{images/hopper_pca.pdf}
\caption{Hopper-v2.}
\end{subfigure}
\hfill
\begin{subfigure}{.45\textwidth}
\centering
\includegraphics[width=0.95\linewidth]{images/walker2d_pca.pdf}
\caption{Walker2d-v2.}
\end{subfigure}
\caption{Visualization of the state coverage for the noisy expert task. According to the experiment set-up, red points correspond to good samples and blue points correspond to noisy and bad samples. Plots show that the state overlap between two modes of samples is large for Hopper-v2 and Walker2d-v2 and is limited for Ant-v2 and HalfCheetah-v2. Therefore, we can expect NBCU performs well on Ant-v2 and HalfCheetah-v2.}
\label{fig:noisy_expert_dataset_coverage}
\end{figure}



\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/noisy_expert_training.pdf}
    \caption{Training curves of BC, DemoDICE \citep{kim2022demodice}, DWBC \citep{xu2022discriminator}, NBCU (\cref{algo:nbcu}), and WBCU (\cref{algo:wbcu}) on the noisy expert task. Solid lines correspond to the mean performance and shaded regions correspond to the 95\% confidence interval. Same as other figures. }
    \label{fig:noisy_expert}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/full_replay_training.pdf}
    \caption{Training curves of BC, DemoDICE \citep{kim2022demodice}, DWBC \citep{xu2022discriminator}, NBCU (\cref{algo:nbcu}), and WBCU (\cref{algo:wbcu}) on the full replay task.}
    \label{fig:full_replay}
\end{figure}





\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/noisy_expert_wbcu.pdf}
    \caption{Training curves of WBCU with gradient penalty on the noisy expert task.}
    \label{fig:noisy_expert_wbcu}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/full_replay_wbcu.pdf}
    \caption{Training curves of WBCU with gradient penalty on the noisy expert task.}
    \label{fig:full_replay_wbcu}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/noisy_expert_demo_dice.pdf}
    \caption{Training curves of DemoDICE with gradient penalty on the full replay task.}
    \label{fig:noisy_expert_demo_dice}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{images/full_replay_demo_dice.pdf}
    \caption{Training curves of DemoDICE with gradient penalty on the full replay task.}
    \label{fig:full_replay_demo_dice}
\end{figure}


==> header.tex <==
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{multirow}    
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{microtype}      %
\usepackage{natbib}
\usepackage{enumerate}
\usepackage{hhline}
\usepackage{makecell}
\usepackage{pifont}

\usepackage{graphicx} %
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{tikz}
\usepackage{xcolor}
\usetikzlibrary{arrows}

\allowdisplaybreaks

\usepackage{mathrsfs}

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{hyperref}
\usepackage{bm}

\allowdisplaybreaks

\newcommand{\RR}{\mathbb{R}}
\newcommand{\vct}{\boldsymbol }
\newcommand{\rnd}{\mathsf}
\newcommand{\ud}{\mathrm d}
\newcommand{\nml}{\mathcal{N}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\hinge}{\mathcal{R}}
\newcommand{\kl}{\mathrm{KL}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\dir}{\mathrm{Dir}}
\newcommand{\mult}{\mathrm{Mult}}
\newcommand{\err}{\mathrm{err}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\acc}{\mathrm{acc}}

\newcommand{\labs}{\left\vert}
\newcommand{\rabs}{\right\vert}
\newcommand{\lnorm}{\left\Vert}
\newcommand{\rnorm}{\right\Vert}

\newcommand{\aff}{\mathrm{aff}}
\newcommand{\Sgn}{\mathrm{sign}}

\newcommand{\hit}{\mathrm{hit}}
\newcommand{\cross}{\mathrm{cross}}
\newcommand{\Left}{\mathrm{left}}
\newcommand{\Right}{\mathrm{right}}
\newcommand{\Mid}{\mathrm{mid}}
\newcommand{\bern}{\mathrm{Bernoulli}}
\newcommand{\ols}{\mathrm{ols}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\unif}{\mathrm{Unif}}
\newcommand{\Image}{\mathrm{im}}
\newcommand{\Kernel}{\mathrm{ker}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\pred}{\mathrm{pred}}
\newcommand{\distequal}{\stackrel{\mathbf{P}}{=}}
\newcommand{\gege}{{A(\vect{w},\vect{w}_*)}}
\newcommand{\gele}{{A(\vect{w},-\vect{w}_*)}}
\newcommand{\lele}{{A(-\vect{w},-\vect{w}_*)}}
\newcommand{\lege}{{A(-\vect{w},\vect{w}_*)}}
\newcommand{\firstlayer}{\mathbf{W}}
\newcommand{\firstlayerWN}{v}
\newcommand{\secondlayer}{a}
\newcommand{\inputvar}{\vect{x}}
\newcommand{\anglemat}{\mathbf{\Phi}}
\newcommand{\holder}{H\"{o}lder }
\newcommand{\real}{\mathbb{R}}
\newcommand{\approxerr}{\delta}

\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cS{\mathcal{S}}
\def\cI{\mathcal{I}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cP{\mathcal{P}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cZ{\mathcal{Z}}
\def\SS{\mathbb{S}}
\def\NN{\mathbb{N}}
\def\bP{\mathbf{P}}
\def\TV{\mathrm{TV}}
\def\MSE{\mathrm{MSE}}

\def\vw{\mathbf{w}}
\def\va{\mathbf{a}}
\def\vZ{\mathbf{Z}}

\newcommand{\mat}[1]{#1}
\newcommand{\vect}[1]{#1}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\normop}[1]{\left\|#1\right\|_{\mathrm{op}}}
\newcommand{\simplex}{\triangle}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\expect}{\mathbb{E}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\proj}{\gP}
\newcommand{\event}[1]{\mathscr{#1}}
\newcommand{\set}[1]{#1}
\newcommand{\diff}{\text{d}}
\newcommand{\difference}{\triangle}
\newcommand{\inputdist}{\mathcal{Z}}
\newcommand{\indict}{\mathbb{I}}
\newcommand{\rotmat}{\mathbf{R}}
\newcommand{\normalize}[1]{\overline{#1}}
\newcommand{\vectorize}[1]{\text{vec}\left(#1\right)}
\newcommand{\vclass}{\mathcal{G}}
\newcommand{\pclass}{\Pi}
\newcommand{\qclass}{\mathcal{Q}}
\newcommand{\rclass}{\mathcal{R}}
\newcommand{\classComplexity}[2]{N_{class}(#1,#2)}
\newcommand{\cclass}{\mathcal{F}}
\newcommand{\gclass}{\mathcal{G}}
\newcommand{\pthres}{p_{thres}}
\newcommand{\ethres}{\epsilon_{thres}}
\newcommand{\eclass}{\epsilon_{class}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\trans}{P}
\newcommand{\lowprobstate}{\psi}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\contexts}{\mathcal{X}}
\newcommand{\edges}{\mathcal{E}}
\newcommand{\variance}{\text{Var}}
\newcommand{\params}{\vect{w}}

\newcommand{\relu}[1]{\sigma\left(#1\right)}
\newcommand{\reluder}[1]{\sigma'\left(#1\right)}
\newcommand{\act}[1]{\sigma\left(#1\right)}

\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{prop}{Proposition}
\newtheorem{asmp}{Assumption}
\newtheorem{defn}{Definition}
\newtheorem{oracle}{Oracle}
\newtheorem{fact}{Fact}
\newtheorem{conj}{Conjecture}
\newtheorem{rem}{Remark}
\newtheorem{example}{Example}
\newtheorem{condition}{Condition}
\newtheorem{exercise}{Exercise}
\newtheorem{mess}{Message}


\usepackage[capitalize,noabbrev]{cleveref}
\crefname{thm}{Theorem}{Theorems}
\crefname{lem}{Lemma}{Lemmas}
\crefname{cor}{Corollary}{Corollaries}
\crefname{prop}{Proposition}{Propositions}
\crefname{asmp}{Assumption}{Assumptions}
\crefname{defn}{Definition}{Definitions}
\crefname{oracle}{Oracle}{Oracles}
\crefname{fact}{Fact}{Facts}
\crefname{conj}{Conjecture}{Conjectures}
\crefname{rem}{Remark}{Remarks}
\crefname{example}{Example}{Examples}
\crefname{condition}{Condition}{Conditions}
\crefname{exercise}{Exercise}{Exercises}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{table}{Table}{Tables}
\crefname{figure}{Figure}{Figures}
\crefname{section}{Section}{Sections}
\crefname{subsection}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\crefname{message}{Message}{Messages}



\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\definecolor{red}{rgb}{1, 0, 0}
\newcommand{\RED}[1]{{\color{red} #1}}

\definecolor{green}{rgb}{0, 1, 0}
\newcommand{\GREEN}[1]{{\bf\color{green} #1}}

\definecolor{blue}{rgb}{0, 0, 1}
\newcommand{\BLUE}[1]{{\color{blue} #1}}

\definecolor{orange}{rgb}{1, 0.4, 0.0}
\newcommand{\ORANGE}[1]{{\color{orange} #1}}



==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{(\ref{#1})}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}



\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ea}{\begin{equation*}}
\newcommand{\eea}{\end{equation*}}

\newcommand{\rar}{\rightarrow}
\newcommand{\lar}{\leftarrow}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left\{}
\newcommand{\rb}{\right\}}
\newcommand{\ls}{\left[}
\newcommand{\rs}{\right]}

\newcommand{\bvec}[1]{\ensuremath{\begin{bmatrix}#1\end{bmatrix}}}
\newcommand{\pvec}[1]{\ensuremath{\begin{pmatrix}#1\end{pmatrix}}}


\let\ab\allowbreak


==> nbcu_results.tex <==
\section{Proof of Results in Section \ref{sec:analysis_of_behavioral_cloning}}

\begin{lem}
\label{lem:binomial_distribution}
For any $N \in \mathbb{N}_{+}$ and $p \in (0, 1)$, if the random variable $X$ follows the binomial distribution, i.e., $X \sim \bin (N, p)$, then we have that
\begin{align*}
    \expect \ls \frac{1}{X+1} \rs \leq \frac{1}{N p}.
\end{align*}
\end{lem}

\begin{proof}
\begin{align*}
    \expect \ls \frac{1}{X+1} \rs &= \sum_{x=0}^N \lp \frac{1}{x+1} \rp  \frac{N!}{x! (N-x)!} p^{x} (1-p)^{N-x}
    \\
    &= \frac{1}{(N+1) p} \sum_{x=1}^{N+1} \lp \frac{(N+1)!}{x! (N+1 - x)!} \rp p^x (1-p)^{N+1-x}
    \\
    &=  \frac{1}{(N+1) p} \lp 1 - (1-p)^{N+1} \rp \leq \frac{1}{N p}. 
\end{align*}
\end{proof}


\subsection{Proof of Theorem \ref{thm:bc_expert}}

When $|\gDE| \geq 1$, by \citep[Theorem 4.2]{rajaraman2020fundamental}, we have that
\begin{align*}
    V(\piE) - \expect_{\gDE} \ls  V(\pi^{\bc}) \rs \leq \frac{4 |\gS| H^2}{9 |\gDE|}.
\end{align*}
When $|\gDE| = 0$, we simply have that
\begin{align*}
    V(\piE) - \expect_{\gDE} \ls  V(\pi^{\bc}) \rs \leq H.
\end{align*}
Therefore, we have the following unified bound.
\begin{align*}
    V(\piE) - \expect_{\gDE} \ls  V(\pi^{\bc}) \rs \leq \frac{|\gS| H^2}{ \max\{ |\gDE|, 1 \}} \leq \frac{2 |\gS| H^2}{ |\gDE|+1}.
\end{align*}
The last inequality follows that $\max\{ x, 1 \} \geq (x + 1)/2, \; \forall x \geq 0$. Finally, notice that $|\gDE| \sim \bin (N_{\tot}, \eta)$. By \cref{lem:binomial_distribution}, we have that
\begin{align*}
     V(\piE) - \expect \ls  V(\pi^{\bc}) \rs \leq \expect \ls \frac{2 |\gS| H^2}{ |\gDE|+1} \rs \leq \frac{2 |\gS| H^2}{ N_{\tot} \eta} = \frac{2 |\gS| H^2}{ N_{\expert} } , 
\end{align*}
which completes the proof.

\subsection{Proof of Theorem \ref{thm:bc_union}}
For analysis, we first define the mixture state-action distribution as follows.
\begin{align*}
     d^{\mix}_h (s, a) \triangleq \eta d^{\piE}_h (s, a) + (1-\eta) d^{\pi^{\beta}}_h (s, a), d^{\mix}_h (s) \triangleq \sum_{a \in \gA} d^{\mix}_h (s, a),  \; \forall (s, a) \in \gS \times \gA, \; \forall h \in [H].   
\end{align*}
Note that in the population level, the marginal state-action distribution of union dataset $\gDU$ in time step $h$ is exactly $d^{\mix}_h$. That is, $d^{\oU}_h (s, a) = d^{\mix}_h (s, a), \; \forall (s, a, h) \in \gS \times \gA \times [H]$. Then we define the mixture policy $\pimix$ induced by $d^{\mix}$ as follows.
\begin{align*}
     \pimix_h (a|s) =
    \begin{cases}
    \frac{d^{\mix}_h (s, a)}{d^{\mix}_h (s) } & \text{if } d^{\mix}_h (s) > 0,
    \\
     \frac{1}{\vert \gA \vert} & \text{otherwise}.
    \end{cases} \; \forall (s, a) \in \gS \times \gA\;, \forall h \in [H].
\end{align*}
From the theory of Markov Decision Processes, we know that (see, e.g., \citep{puterman2014markov}) 
\begin{align*}
    \forall h \in [H], \forall (s, a) \in \gS \times \gA, d^{\pimix}_h (s, a) = d^{\mix}_h (s, a). 
\end{align*}
Therefore, we can obtain that the marginal state-action distribution of union dataset $\gDU$ in time step $h$ is exactly $d^{\pimix}_h$. Then we have the following decomposition.
\begin{align*}
    \expect \ls V(\piE) - V(\pi^{\nbcu}) \rs &= \expect \ls V(\piE) - V (\pimix) +  V (\pimix) -  V(\pi^{\nbcu}) \rs
    \\
    &= \expect \ls V(\piE) - V (\pimix) \rs + \expect \ls  V (\pimix) -  V(\pi^{\nbcu}) \rs
    \\
    &= V(\piE) - V (\pimix) + \expect \ls  V (\pimix) -  V(\pi^{\nbcu}) \rs.  
\end{align*}
For $V(\piE) - V (\pimix)$, we have that 
\begin{align*}
    V(\piE) - V (\pimix) &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \lp d^{\piE}_h (s, a) - d^{\pimix}_h (s, a) \rp r_h (s, a)
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \lp d^{\piE}_h (s, a) - d^{\mix}_h (s, a) \rp r_h (s, a) 
    \\
    &= (1-\eta) \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \lp d^{\piE}_h (s, a) - d^{\pi^{\beta}}_h (s, a) \rp r_h (s, a)
    \\
    &= (1-\eta) \lp V (\piE) - V (\pi^{\beta}) \rp.
\end{align*}
The last equation follows the dual formulation of policy value \citep{puterman2014markov}. Besides, notice that $\expect \ls  V (\pimix) -  V(\pi^{\nbcu}) \rs$ is exactly the imitation gap of BC when regarding $\pimix$ and $\gDU$ as the expert policy and expert demonstrations, respectively. By \citep[Theorem 4.4]{rajaraman2020fundamental}, we have that
\begin{align*}
    \expect \ls  V (\pimix) -  V(\pi^{\nbcu})  \rs \lesssim  \frac{|\gS| H^2 \log (N_{\tot})}{N_{\tot}}.
\end{align*}
Combining the above two equations yields that
\begin{align*}
    \expect \ls V(\piE) - V(\pi^{\nbcu}) \rs \lesssim (1-\eta) \lp V (\piE) - V (\pi^{\beta}) \rp + \frac{|\gS| H^2 \log (N_{\tot})}{N_{\tot}}. 
\end{align*}


\subsection{Proof of Proposition \ref{prop:bc_union_lower_bound}}

We consider the instance named Standard Imitation in \citep{xu2021error}; see \cref{fig:standard_imitation}. In Standard Imitation, each state is an absorbing state. In each state, only by taking the action $a^1$, the agent can obtain the reward of $1$. Otherwise, the agent obtains zero rewards. The initial state distribution is a uniform distribution, i.e., $\rho (s) = 1/|\gS|, \forall s \in \gS$. 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\linewidth]{images/Standard_Imitation.pdf}
    \caption{The Standard Imitation MDP in \citep{xu2021error}.}
    \label{fig:standard_imitation}
\end{figure}



We consider that the expert policy $\piE$ always takes the action $a^1$ while the behavioral policy $\pi^{\beta}$ always takes another action $a^2$. Formally, $\piE_h (a^1|s) = 1, \forall s \in \gS, h \in [H], \; \pi^{\beta}_h (a^2|s) = 1, \forall s \in \gS, h \in [H]$. It is direct to calculate that $V (\piE) = H$ and $V (\pi^{\beta}) = 0$. The supplementary dataset $\gDS$ and the expert dataset $\gDE$ are collected according to \cref{asmp:dataset_collection}. The mixture state-action distribution can be calculated as $\forall s \in \gS, h \in [H]$,
\begin{align*}
    & d^{\mix}_h (s, a^1) = \eta d^{\piE}_h (s, a^1) + (1-\eta) d^{\pi^{\beta}}_h (s, a^1) = \eta d^{\piE}_h (s, a^1) = \eta \rho (s),
    \\
    & d^{\mix}_h (s, a^2) = \eta d^{\piE}_h (s, a^2) + (1-\eta) d^{\pi^{\beta}}_h (s, a^2) = (1-\eta) d^{\pi^{\beta}}_h (s, a^2) = (1-\eta) \rho (s).  
\end{align*}
Note that in the population level, the marginal distribution of the union dataset $\gDU$ in time step $h$ is exactly $d^{\mix}_h$. The mixture policy induced by $d^{\mix}$ can be formulated as
\begin{align*}
\pimix_h (a^1|s) = \eta, \pimix_h (a^2|s) = 1-\eta, \forall s \in \gS, h \in [H]. 
\end{align*}
Just like before, we have $d^{\pimix}_h (s, a) = d^{\mix}_h (s, a)$. The policy value of $\pimix$ can be calculated as 
\begin{align*}
    V (\pimix) = \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} d^{\mix}_h (s, a) r_h (s, a) = \sum_{h=1}^H \sum_{s \in \gS} d^{\mix}_h (s, a^1) = \eta H.  
\end{align*}
The policy $\pi^{\nbcu}$ can be formulated as
\begin{align}
 \forall h \in [H], \quad    \pi^{\nbcu}_h(a|s) = \left\{ \begin{array}{ll}
      \frac{n^{\oU}_h(s, a)}{\sum_{a^\prime} n^{\oU}_h(s, a^\prime)}  & \text{if}\sum_{a^\prime} n^{\oU}_h(s, a^\prime) > 0  \\
        \frac{1}{|\gA|} & \text{otherwise}  
    \end{array} \right.
\end{align}
We can view that the BC's policy learned on the union dataset mimics the mixture policy $\pimix$. In the following part, we analyze the lower bound on the imitation gap of $\pi^{\nbcu}$.
\begin{align*}
    \expect \ls V (\piE) - V (\pibcunion) \rs &= V (\piE) - V (\pimix) + \expect \ls V (\pimix) - V (\pibcunion)  \rs
    \\
    &= H - \eta H + \expect \ls V (\pimix) - V (\pibcunion)  \rs
    \\
    &= (1-\eta) (V (\piE) - V (\pi^\beta)) + \expect \ls V (\pimix) - V (\pibcunion)  \rs. 
\end{align*}
Then we consider the term $\expect \ls V (\pimix) - V (\pibcunion)  \rs$.
\begin{align*}
     V (\pimix) - V (\pibcunion) &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \lp d^{\pimix}_h (s, a) - d^{\pibcunion}_h (s, a) \rp r_h (s, a)
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a)
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a) \indict \{ n^{\oU}_h (s) > 0  \}
    \\
    &\quad + \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a) \indict \{ n^{\oU}_h (s) = 0  \}. 
\end{align*}
We take expectation over the randomness in $\gDU$ on both sides and obtain that
\begin{align}
\expect \ls V (\pimix) - V (\pibcunion) \rs  &= \expect \ls \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a) \indict \{ n^{\oU}_h (s) > 0  \} \rs \nonumber
    \\
    &\quad + \expect \ls \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a) \indict \{ n^{\oU}_h (s) = 0  \} \rs. \label{eq:lower_bound_decomposition} 
\end{align}
For the first term in RHS, we have that
\begin{align*}
    &\quad \expect \ls \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a) \indict \{ n^{\oU}_h (s) > 0  \} \rs
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) r_h (s, a) \expect \ls  \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp \indict \{ n^{\oU}_h (s) > 0  \} \rs
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) r_h (s, a) \sP \lp n^{\oU}_h (s) > 0 \rp \expect \ls  \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp \bigg|  n^{\oU}_h (s) > 0  \rs
    \\
    &= 0.
\end{align*}
The last equation follows the fact that when $n^{\oU}_h (s) > 0$, $\pibcunion_h (a|s)$ is an unbiased maximum likelihood estimation of $\pimix_h (a|s)$. For the remaining term, we have that
\begin{align*}
    &\quad \expect \ls \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a) \indict \{ n^{\oU}_h (s) = 0  \} \rs
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) r_h (s, a) \expect \ls   \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp  \indict \{ n^{\oU}_h (s) = 0  \} \rs
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) r_h (s, a) \sP \lp n^{\oU}_h (s) = 0 \rp \expect \ls   \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp \bigg| n^{\oU}_h (s) = 0 \rs
    \\
    &= \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) r_h (s, a) \sP \lp n^{\oU}_h (s) = 0 \rp \lp \pi^{\mix}_h (a|s) - \frac{1}{\vert \gA \vert} \rp
    \\
    &\overset{(a)}{=} \sum_{h=1}^H \sum_{s \in \gS} \rho (s) \sP \lp n^{\oU}_h (s) = 0 \rp \lp \eta - \frac{1}{\vert \gA \vert} \rp
    \\
    & \overset{(b)}{=} H \lp \eta - \frac{1}{\vert \gA \vert} \rp \sum_{s \in \gS} \rho (s) \sP \lp n^{\oU}_1 (s) = 0 \rp. 
\end{align*}
In the equation $(a)$, we use the fact that $r_h (s, a^1) = 1, r_h (s, a) = 0, \forall a \in \gA \setminus \{a^1 \}$. In the equation $(b)$, since each state is an absorbing state, we have that $\sP \lp n^{\oU}_h (s) = 0 \rp = \sP \lp n^{\oU}_1 (s) = 0 \rp, \forall h \in [H]$.


We consider two cases. In the first case of $\eta \geq 1/\vert \gA \vert$, we directly have that
\begin{align*}
    \expect \ls \sum_{h=1}^H \sum_{(s, a) \in \gS \times \gA} \rho (s) \lp \pimix_h (a|s) - \pibcunion_h (a|s) \rp r_h (s, a) \indict \{ n^{\oU}_h (s) = 0  \} \rs \geq 0.
\end{align*}
By \cref{eq:lower_bound_decomposition}, we have that
\begin{align*}
    \expect \ls V (\pimix) - V (\pibcunion) \rs \geq 0,
\end{align*}
which implies that
\begin{align*}
    \expect \ls V (\piE) - V (\pibcunion) \rs \geq  (1-\eta) (V (\piE) - V (\pi^\beta)).
\end{align*}
In the second case of $\eta < 1/\vert \gA \vert$, we have that
\begin{align*}
     H \lp \eta - \frac{1}{\vert \gA \vert} \rp \sum_{s \in \gS} \rho (s) \sP \lp n^{\oU}_1 (s) = 0 \rp
    &\overset{(a)}{\geq} - \lp \frac{1}{\vert \gA \vert} - \eta \rp H \exp \lp - \frac{N_{\tot}}{|\gS|} \rp
    \\
    &\geq - (1-\eta) H \exp \lp - \frac{N_{\tot}}{|\gS|} \rp
    \\
    &\overset{(b)}{\geq} -\frac{ (1-\eta) H}{2}.
\end{align*}
In the inequality $(a)$, we use that 
\begin{align*}
    \sum_{s \in \gS} \rho (s) \sP \lp n^{\oU}_1 (s) = 0 \rp = \sum_{s \in \gS} \rho (s) (1-\rho (s))^{N_{\tot}} = \lp 1-\frac{1}{\vert \gS \vert} \rp^{N_{\tot}} \leq \exp \lp - \frac{N_{\tot}}{\vert \gS \vert} \rp.
\end{align*}
The inequality $(b)$ holds since we consider the range where $N_{\tot} \geq \vert \gS \vert \log (2) $. By \cref{eq:lower_bound_decomposition}, we have that
\begin{align*}
    \expect \ls V (\pimix) - V (\pibcunion) \rs \geq - \frac{ (1-\eta) H}{2}.
\end{align*}
This implies that
\begin{align*}
    \expect \ls V (\piE) - V (\pibcunion) \rs &\geq  (1-\eta) (V (\piE) - V (\pi^\beta)) - \frac{(1-\eta) H}{2}
    \\
    &=  \frac{(1-\eta)}{2} (V (\piE) - V (\pi^\beta)). 
\end{align*}
In both cases, we prove that $\expect \ls V (\piE) - V (\pibcunion) \rs \gtrsim (1-\eta) (V (\piE) - V (\pi^\beta)) $ and thus complete the proof.



\subsection{Proof of Theorem \ref{thm:bc_imitation_gap_expert}}
When $\pi^\beta = \piE$, $\expect \ls V (\piE) - V (\pibcunion) \rs$ is exactly the imitation gap of BC on $\gDU$ with expert policy $\piE$.  By \citep[Theorem 4.2]{rajaraman2020fundamental}, we finish the proof.


\subsection{Proof of Theorem \ref{thm:bc_imitation_gap_no_overlap}}

According to the policy difference lemma in \citep{kakade2002pg}, we have that
\begin{align*}
    V (\piE) - V (\pibcunion) &= \sum_{h=1}^H \expect_{s_h \sim d^{\piE}_h (\cdot)} \ls Q^{\pibcunion}_h (s_h, \piE_h (s_h)) - \sum_{a \in \gA} \pibcunion_h (\cdot|s_h) Q^{\pibcunion}_h (s_h, a)  \rs
    \\
    &= \sum_{h=1}^H \expect_{s_h \sim d^{\piE}_h (\cdot)} \ls Q^{\pibcunion}_h (s_h, \piE_h (s_h)) (1-\pibcunion_h (\piE_h (s_h)|s_h))  \rs  
    \\
    &\leq H \sum_{h=1}^H \expect_{s \sim d^{\piE}_h (\cdot)} \ls \expect_{a \sim \pibcunion_h (\cdot|s)} \ls \indict \lb a \not= \piE_h (s) \rb \rs \rs,
\end{align*}
where $Q^{\pi}_h(s, a) = \expect[\sum_{t=h}^{H} r(s_t, a_t) |(s_h, a_h) = (s, a)]$ is the state-action value function for a policy $\pi$ and $\piE_h(s_h)$ denotes the expert action. By assumption, we have $\forall h \in [H]$, $\supp (d^{\piE}_h (\cdot)) \cap \supp (d^{\pi^{\beta}}_h (\cdot)) = \emptyset$. Therefore, we know that the union state-action pairs in $\gDU$ does not affect $\pibcunion$ on expert states. As a result, $\pibcunion$ exactly takes expert actions on states visited in $\gDE$. Then we have that
\begin{align*}
    V (\piE) - V (\pibcunion) \leq H \sum_{h=1}^H \expect_{s \sim d^{\piE}_h (\cdot)} \ls \indict \lb s \notin \gS_h (\gDE) \rb \rs,
\end{align*}
where $\gS_h (\gDE)$ is the set of states in time step $h$ in $\gDE$. Taking expectation over the randomness within $\gDE$ on both sides yields that
\begin{align*}
    V (\piE) - \expect_{\gDE} \ls V (\pibcunion) \rs \leq H \expect_{\gDE} \ls \sum_{h=1}^H \expect_{s \sim d^{\piE}_h (\cdot)} \ls \indict \lb s \notin \gS_h (\gDE) \rb \rs \rs.
\end{align*}
By \citep[Lemma A.1]{rajaraman2020fundamental}, we further derive that
\begin{align*}
    V (\piE) - \expect_{\gDE} \ls V (\pibcunion) \rs \leq  \frac{|\gS| H^2}{ \max \{ |\gDE|, 1\}} \leq  \frac{2 |\gS| H^2}{ |\gDE|+ 1}. 
\end{align*}
We take expectation over the binomial variable $|\gDE|$ and have that
\begin{align*}
    V (\piE) - \expect \ls V (\pibcunion) \rs \leq \expect \ls \frac{2 |\gS| H^2}{ |\gDE|+ 1} \rs \leq \frac{2 |\gS| H^2}{N_{\tot} \eta} = \frac{2 |\gS| H^2}{N_{\expert}} , 
\end{align*}
which completes the proof.



==> packages/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{(\ref{#1})}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}



\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\newcommand{\e}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ea}{\begin{equation*}}
\newcommand{\eea}{\end{equation*}}

\newcommand{\rar}{\rightarrow}
\newcommand{\lar}{\leftarrow}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lb}{\left\{}
\newcommand{\rb}{\right\}}
\newcommand{\ls}{\left[}
\newcommand{\rs}{\right]}

\newcommand{\bvec}[1]{\ensuremath{\begin{bmatrix}#1\end{bmatrix}}}
\newcommand{\pvec}[1]{\ensuremath{\begin{pmatrix}#1\end{pmatrix}}}


\let\ab\allowbreak


==> technical_lemma.tex <==
  

==> wbcu_results.tex <==
\section{Proof of Results in Section \ref{sec:analysis_of_weighted_behavioral_cloning}}
\label{sec:proof_of_weighted_behavioral_cloning}

\subsection{Proof of Proposition \ref{prop:wbcu_negative}}


In the tabular case, with the first-order optimality condition, we have $c^\star_h (s, a) = \widehat{d^{\expert}_h} (s, a) /( \widehat{d^{\expert}_h} (s, a) + \widehat{d^{\oU}_h} (s, a)) $. By \cref{eq:from_c_to_w}, we have 
\begin{align*}
   \widehat{d^{\oU}_h}(s, a) w_h(s, a) =  \widehat{d^{\oU}_h}(s, a)  \times \frac{\widehat{d^{\expert}_h} (s, a)}{\widehat{d^{\oU}_h} (s, a)} = \widehat{d^{\expert}_h}(s, a). 
\end{align*}
Hence, the learning objective \eqref{eq:weighted_bc} reduces to \eqref{eq:bc_opt}.


\subsection{Proof of Lemma \ref{lem:lipschitz_continuity}}
Recall that
\begin{align*}
    \Delta_h(\theta)= \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}   \langle  \theta,  \phi_h (s, a) \rangle - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \langle  \theta,  \phi_h (s^\prime, a^\prime) \rangle.
\end{align*}
Then we have that
\begin{align*}
 \Delta_h(\bar{\theta}_h)  - \Delta_h(\theta) &= \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}   \langle  \bar{\theta}_h,  \phi_h (s, a) \rangle - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \langle  \bar{\theta}_h,  \phi_h (s^\prime, a^\prime) \rangle
 \\
 &\quad - \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}   \langle  \theta,  \phi_h (s, a) \rangle + \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \langle  \theta,  \phi_h (s^\prime, a^\prime) \rangle
 \\
 &\overset{(a)}{\leq} \langle  \bar{\theta}_h,  \phi_h (s^1, a^1) \rangle - \langle  \bar{\theta}_h,  \phi_h (s^2, a^2) \rangle -   \langle  \theta,  \phi_h (s^1, a^1) \rangle +  \langle  \theta,  \phi_h (s^2, a^2) \rangle
 \\
 &= \langle \bar{\theta}_h - \theta, \phi_h (s^1, a^1) - \phi_h (s^2, a^2)   \rangle
 \\
 &\overset{(b)}{\leq} \lnorm \bar{\theta}_h - \theta \rnorm \lnorm \phi_h (s^1, a^1) - \phi_h (s^2, a^2) \rnorm.
\end{align*}
In inequality $(a)$, we utilize the facts that $(s^1, a^1) \in \argmin_{ (s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \langle \theta_h,  \phi_h (s, a) \rangle$ and \\ $(s^2, a^2) \in \argmax_{(s, a) \in  \gD^{\oS, 2}_h } \langle \theta_h,  \phi_h (s, a) \rangle$. Inequality $(b)$ follows the Cauchy–Schwarz inequality. Let $L_h = \lnorm \phi_h (s^1, a^1) - \phi_h (s^2, a^2) \rnorm$ and we finish the proof.

\subsection{Proof of Lemma \ref{lem:strong_convexity}}
First, by Taylor's Theorem, there exists $\theta_h^\prime \in \{ \theta \in \reals^d: \theta^t = \theta^\star_h + t (\widebar{\theta}_h - \theta^\star_h), \; \forall t \in [0, 1] \}$ such that
\begin{align}
    \gL_h (\widebar{\theta}_h) &= \gL_h (\theta^\star_h) + \langle \nabla \gL_h (\theta^\star_h), \widebar{\theta}_h - \theta^\star_h   \rangle + \frac{1}{2} \lp \widebar{\theta}_h - \theta^\star_h \rp^\top \nabla^2 \gL_h (\theta_h^\prime) \lp \widebar{\theta}_h - \theta^\star_h \rp \nonumber
    \\
    &= \gL_h (\theta^\star_h) + \frac{1}{2} \lp \widebar{\theta}_h - \theta^\star_h \rp^\top \nabla^2 \gL_h (\theta_h^\prime) \lp \widebar{\theta}_h - \theta^\star_h \rp. \label{eq:taylor_approximation}
\end{align}
The last equality follows the optimality condition that $\nabla \gL_h (\theta^\star_h) = 0$. Then, our strategy is to prove that the smallest eigenvalue of the Hessian matrix $\nabla^2 \gL_h (\theta_h^\prime)$ is positive, i.e., $\lambda_{\min} (\nabla^2 \gL_h (\theta_h^\prime)) > 0$. We first calculate the Hessian matrix $\nabla^2 \gL_h (\theta_h^\prime)$. Given $\gDE$ and $\gDU$, we define the function $G: \reals^{(|\gDE| + |\gDU|)} \rightarrow \reals$ as
\begin{align*}
    G (v) \triangleq \frac{1}{|\gDE|} \sum_{i=1}^{|\gDE|} g (v_i) + \frac{1}{|\gDU|} \sum_{j=1}^{|\gDU|} g (v_j),  
\end{align*}
where $v_i$ is the $i$-th element in the vector $v \in \reals^{(|\gDE| + |\gDU|)}$ and $g (x) = \log \lp 1 + \exp (x) \rp $ is a real-valued function. Besides, we use $B_h \in \reals^{ (|\gDE| + |\gDU|) \times d}$ to denote the matrix whose $i$-th row $B_{h, i} = - y_i \phi_h (s^i, a^i)^\top$, and $y_i = 1$ if $ (s^i, a^i) \in \gDE_h$, $y_i = -1$ if $ (s^i, a^i) \notin \gDE_h$. Then the objective function can be reformulated as
\begin{align*}
\gL_h (\theta_h) &= \sum_{(s, a)} \widehat{d^{\expert}_h}(s, a) \ls \log \lp 1 + \exp \lp - \langle \phi_h (s,a), \theta_h \rangle \rp \rp \rs + \sum_{(s, a)} \widehat{d^{\oU}_h} (s, a) \ls \log \lp 1 + \exp \lp \langle \phi_h (s,a), \theta_h \rangle \rp \rp \rs
\\
&= \frac{1}{|\gDE|} \sum_{(s, a) \in \gDE} \log \lp 1 + \exp \lp - \langle \phi_h (s,a), \theta_h \rangle \rp \rp + \frac{1}{|\gDU|} \sum_{(s, a) \in \gDU} \log \lp 1 + \exp \lp \langle \phi_h (s,a), \theta_h \rangle \rp \rp  
\\
&= G (B_h \theta_h).
\end{align*}
Then we have that $\nabla^2 \gL_h (\theta_h) = B_h^\top \nabla^2 G (B_h \theta_h) B_h$, where
\begin{align*}
     \nabla^2 G (B_h \theta_h) = \diag \lp \frac{g^{\prime \prime} ((B_h \theta_h)_1)}{|\gDE|}, \ldots, \frac{g^{\prime \prime} ((B_h \theta_h)_{|\gDE|})}{|\gDE|}, \frac{g^{\prime \prime} ((B_h \theta_h)_{|\gDE| + 1})}{|\gDE |+ |\gDU|}, \ldots, \frac{g^{\prime \prime} ((B_h \theta_h)_{|\gDE |+ |\gDU|})}{|\gDE |+ |\gDU|}    \rp.
\end{align*}
Here $g^{\prime \prime} (x) = \sigma (x) (1-\sigma (x))$, where $\sigma (x) = 1/(1+\exp (-x))$ is the sigmoid function. The eigenvalues of $\nabla^2 G (B_h \theta_h)$ are
\begin{align*}
    \lb \frac{g^{\prime \prime} ((B_h \theta_h)_1)}{|\gDE|}, \ldots, \frac{g^{\prime \prime} ((B_h \theta_h)_{|\gDE|})}{|\gDE|}, \frac{g^{\prime \prime} ((B_h \theta_h)_{|\gDE| + 1})}{|\gDE |+ |\gDU|}, \ldots, \frac{g^{\prime \prime} ((B_h \theta_h)_{|\gDE |+ |\gDU|})}{|\gDE |+ |\gDU|} \rb.
\end{align*}
Notice that $\theta_h^\prime \in \{ \theta \in \reals^d: \theta^t = \theta^\star_h + t (\widebar{\theta}_h - \theta^\star_h), \; \forall t \in [0, 1] \}$. For a matrix $A$, we use $\lambda_{\min} (A)$ to denote the minimal eigenvalue of $A$. Here we claim that the minimum of the minimal eigenvalues of $\nabla^2 G (B_h \theta^t)$ over $t \in [0, 1]$ is achieved at $t=0$ or $t=1$. That is,
\begin{align*}
    \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^t)) : \forall t \in [0, 1] \} = \min \{\lambda_{\min} ( \nabla^2 G (B_h \theta^0)), \lambda_{\min} ( \nabla^2 G (B_h \theta^1))  \}.
\end{align*}
We prove this claim as follows. For any $t \in [0, 1]$, we use $\{ \lambda_1 (t), \ldots,  \lambda_{|\gDE| + |\gDU|} (t)\}$ to denote the eigenvalues of $\nabla^2 G (B_h \theta^t)$. For each $i \in [|\gDE| + |\gDU|]$, we consider $\lambda_i (t) :[0, 1] \rightarrow \reals$ as a function of $t$. Specifically,
\begin{align*}
    \lambda_{i} (t) = \begin{cases}
    \frac{g^{\prime \prime} ((B_h \theta^\star_h)_{i} + t (B_h (\widebar{\theta}_h - \theta^\star_h))_{i})}{|\gDE|}, &\quad \text{if } i \in [|\gDE|]
    \\
    \frac{g^{\prime \prime} ((B_h \theta^\star_h)_{i} + t (B_h (\widebar{\theta}_h - \theta^\star_h))_{i})}{|\gDE| + |\gDU|}, &\quad \text{otherwise}.
    \end{cases}
\end{align*}
We observe that $g^{\prime \prime \prime} (x) = \sigma (x) (1-\sigma (x)) (1-2\sigma (x))$ which satisfies that $ \forall x \leq 0, \; g^{\prime \prime \prime} (x) \geq 0, $ and $\forall x \geq 0, \; g^{\prime \prime \prime} (x) \leq 0 $. Therefore, we have that the minimum of $\lambda_i (t)$ over $t \in [0, 1]$ must be achieved at $t=0$ or $t=1$. That is,
\begin{align}
\label{eq:min_eigenvalues_boundary}
    \min_{t \in [0, 1]} \lambda_i (t) = \min \{ \lambda_i (0), \lambda_i (1) \}.
\end{align}



For any $t \in [0, 1]$, we define $i^t \in [|\gDE| + |\gDU|]$ as the index of the minimal eigenvalue of $\nabla^2 G (B_h \theta^t)$, i.e., $\lambda_{i^t} (t) = \lambda_{\min} (\nabla^2 G (B_h \theta^t))$. Then we have that
\begin{align*}
    \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^t)) : \forall t \in [0, 1] \} &= \min \{ \lambda_{i^t} (t): \forall t \in [0, 1] \}
    \\
    &\overset{(a)}{=} \min \{ \min \{ \lambda_{i^t} (0), \lambda_{i^t} (1 ) \}: \forall t \in [0, 1] \}
    \\
    &= \min \{ \lambda_{i^0} (0), \lambda_{i^1} (1) \}
    \\
    &\overset{(b)}{=} \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^0)), \lambda_{\min} (\nabla^2 G (B_h \theta^1)) \} 
\end{align*}
Equality $(a)$ follows \eqref{eq:min_eigenvalues_boundary} and equality $(b)$ follows that $\lambda_{i^0} (0)$ and $\lambda_{i^1} (1)$ are the minimal eigenvalues of $\nabla^2 G (B_h \theta^0)$ and $\nabla^2 G (B_h \theta^1)$, respectively.



In summary, we derive that
\begin{align}
\label{eq:minimal_eigenvalue}
    \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^t)) : \forall t \in [0, 1] \} = \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^0)), \lambda_{\min} (\nabla^2 G (B_h \theta^1)) \},
\end{align}
which proves the previous claim.






Further, we consider $\lambda_{\min} \lp \nabla^2 \gL_h (\theta_h)  \rp$.
\begin{align*}
    \lambda_{\min} \lp \nabla^2 \gL_h (\theta_h)  \rp &= \inf_{x \in \reals^d: \lnorm x \rnorm = 1} x^\top  \nabla^2 \gL_h (\theta_h) x
    \\
    &= \inf_{x \in \reals^d: \lnorm x \rnorm = 1} \lp B_h x \rp^\top  \nabla^2 G (B_h \theta_h) \lp B_h x \rp
    \\
    &= \inf_{z \in \operatorname{Im} (B_h)} z^\top \nabla^2 G (B_h \theta_h) z
    \\
    &= \lp \inf_{z \in \operatorname{Im} (B_h)} \lnorm z \rnorm \rp^2 \lambda_{\min} (\nabla^2 G (B_h \theta_h))
    \\
    &\geq \lp \inf_{z \in \operatorname{Im} (B_h)} \lnorm z \rnorm \rp^2 \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^0)), \lambda_{\min} (\nabla^2 G (B_h \theta^1)) \}. 
\end{align*}
Here $\operatorname{Im} (B_h) = \{ z \in \reals^d: z = B_h x, \lnorm x \rnorm = 1 \}$. The last inequality follows \cref{eq:minimal_eigenvalue}. 



In the under-parameterization case where $\rank (A_h) = d$, we have that $\rank (B_h) = d$. Thus, $\operatorname{Im} (B_h)$ is a set of vectors with positive norms, i.e., $ \inf_{z \in \operatorname{Im} (B_h)} \lnorm z \rnorm > 0$. Besides, since $g^{\prime \prime} (x) = \sigma (x) (1-\sigma (x)) > 0$, we also have that 
\begin{align*}
    \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^0)), \lambda_{\min} (\nabla^2 G (B_h \theta^1)) \} > 0.
\end{align*}
In summary, we obtain that
\begin{align*}
    \lambda_{\min} \lp \nabla^2 \gL_h (\theta_h)  \rp \geq \lp \inf_{z \in \operatorname{Im} (B_h)} \lnorm z \rnorm \rp^2 \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^0)), \lambda_{\min} (\nabla^2 G (B_h \theta^1)) \} > 0. 
\end{align*}
Then, with \cref{eq:taylor_approximation}, there exists $\tau_h = \lp \inf_{z \in \operatorname{Im} (B_h)} \lnorm z \rnorm \rp^2 \min \{ \lambda_{\min} (\nabla^2 G (B_h \theta^0)), \lambda_{\min} (\nabla^2 G (B_h \theta^1)) \} > 0$ such that
\begin{align*}
    \gL_h (\widebar{\theta}_h) \geq \gL_h (\theta^\star_h) + \frac{\tau_h}{2} \lnorm \widebar{\theta}_h - \theta^\star_h \rnorm^2,
\end{align*}
which completes the proof.


\subsection{Proof of Theorem \ref{thm:wbcu}}
First, invoking \cref{lem:lipschitz_continuity} with $\theta = \theta^\star_h$ yields that
\begin{align*}
    \Delta_h(\theta^\star_h)  \geq \Delta_h(\bar{\theta}_h)  - L_h \lnorm \bar{\theta}_h - \theta^\star_h \rnorm.
\end{align*}
Here $L_h = \lnorm \phi_h (s, a) - \phi_h (s^\prime, a^\prime) \rnorm$ with $(s, a) \in \argmin_{ (s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \langle \theta^\star_h,  \phi_h (s, a) \rangle$ and \\ $(s^\prime, a^\prime) \in \argmax_{(s, a) \in  \gD^{\oS, 2}_h } \langle \theta^\star_h, \phi_h (s, a) \rangle$. Then, by \cref{lem:strong_convexity}, there exists $\tau_h > 0$ such that 
\begin{align*}
    \gL_h (\widebar{\theta}_h) \geq \gL_h (\theta^\star_h) + \frac{\tau_h}{2} \lnorm \widebar{\theta}_h - \theta^\star_h \rnorm^2.
\end{align*}
This directly implies an upper bound of the distance between $\widebar{\theta}_h$ and $\theta^\star_h$. 
\begin{align*}
    \lnorm \widebar{\theta}_h - \theta^\star_h \rnorm \leq \sqrt{ \frac{2 \lp \gL_h(\bar{\theta}_h) - \gL_h(\theta^{\star}_h) \rp}{\tau_h}}.
\end{align*}
When inequality $\eqref{eq:condition}$ holds, we further have that $\lnorm \widebar{\theta}_h - \theta^\star_h \rnorm < \Delta_h (\bar{\theta}_h) / L_h$. Then we get that
\begin{align*}
    \Delta_h(\theta^\star_h)  \geq \Delta_h(\bar{\theta}_h)  - L_h \lnorm \bar{\theta}_h - \theta^\star_h \rnorm >0,
\end{align*}
which completes the proof.

\subsection{An Example Corresponding to Theorem \ref{thm:wbcu}}
\begin{example}
\label{example:condition}
To illustrate \cref{thm:wbcu}, we consider an example in the feature space $\reals^2$. In particular, for time step $h \in [H]$, we have the expert dataset and supplementary dataset as follows.
\begin{align*}
    &\gDE_h = \lb \lp s^{(1)}, a^{(1)} \rp,  \lp s^{(4)}, a^{(4)} \rp \rb, \; \gDS_h = \lb \lp s^{(2)}, a^{(2)} \rp, \lp s^{(3)}, a^{(3)} \rp  \rb, \; \\
    &\gD^{\oS, 1}_h = \lb \lp s^{(2)}, a^{(2)} \rp \rb, \; \gD^{\oS, 2}_h = \lb \lp s^{(3)}, a^{(3)} \rp \rb.
\end{align*}
The corresponding features are
\begin{align*}
    &\phi_h \lp s^{(1)}, a^{(1)} \rp = (0, 1)^\top ,\;  \phi_h \lp s^{(2)}, a^{(2)} \rp = \lp - \frac{1}{2}, 0 \rp^\top, \\
    &\phi_h \lp s^{(3)}, a^{(3)} \rp = \lp 0, -\frac{1}{2} \rp^\top, \; \phi_h \lp s^{(4)}, a^{(4)} \rp = (-1, 0)^\top.
\end{align*}
Notice that the set of expert-style samples is $\gDE_h \cup \gD^{\oS, 1}_h = \{ ( s^{(1)}, a^{(1)} ), ( s^{(2)}, a^{(2)} ),  ( s^{(4)}, a^{(4)} ) \}$ and the set of non-expert-style samples is $\gD^{\oS, 2}_h = \{  ( s^{(3)}, a^{(3)} ) \}$. It is direct to calculate that the ground-truth parameter that achieves the maximum margin among unit vectors is $\widebar{\theta}_h = (-\sqrt{2}/2, \sqrt{2}/2)^\top$ and the maximum margin is $\Delta_h (\widebar{\theta}_h) = \sqrt{2}/2$. According to \cref{eq:parameterized_discriminator_opt}, for $\theta_h = (\theta_{h, 1}, \theta_{h, 2})^\top$, the optimization objective is 
\begin{align*}
    \gL_h (\theta_h) &= \sum_{(s, a)} \widehat{d^{\expert}_h}(s, a) \ls \log \lp 1 + \exp \lp - \langle \phi_h (s,a), \theta_h \rangle \rp \rp \rs + \sum_{(s, a)} \widehat{d^{\oU}_h} (s, a) \ls \log \lp 1 + \exp \lp \langle \phi_h (s,a), \theta_h \rangle \rp \rp \rs
    \\
    &=  \frac{1}{2} \lp \log \lp 1 + \exp \lp - \theta_{h, 2} \rp \rp + \log \lp 1 + \exp \lp \theta_{h, 1} \rp \rp  \rp 
    \\
    & \quad + \frac{1}{4} \lp \log \lp 1 + \exp \lp  \theta_{h, 2} \rp \rp + \log \lp 1 + \exp \lp - \frac{1}{2}  \theta_{h, 1} \rp \rp \rp \\
    &\quad + \frac{1}{4} \lp \log \lp 1 + \exp \lp -\frac{1}{2}  \theta_{h, 2} \rp \rp + \log \lp 1 + \exp \lp  - \theta_{h, 1} \rp \rp  \rp. 
\end{align*}
We apply CVXPY \citep{diamond2016cvxpy} to calculate the optimal solution $\theta^\star_h \approx (-0.310, 0.993)^\top$ and the objective values $\gL_h (\theta^\star_h) \approx 1.287, \; \gL_h (\widebar{\theta}_h) \approx 1.309 $. Furthermore, we calculate the Lipschitz coefficient $L_h$ appears in \cref{lem:lipschitz_continuity}.
\begin{align*}
    & (s^{(2)}, a^{(2)})  = \argmin_{ (s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \langle \theta^\star_h,  \phi_h (s, a) \rangle , \; (s^{(3)}, a^{(3)}) \in \argmax_{(s, a) \in  \gD^{\oS, 2}_h } \langle \theta^\star_h,  \phi_h (s, a) \rangle,
    \\
    & L_h = \lnorm \phi_h (s^{(2)}, a^{(2)}) - \phi_h (s^{(3)}, a^{(3)}) \rnorm = \frac{\sqrt{2}}{2}.  
\end{align*}
Then we calculate the parameter of strong convexity $\tau_h$ appears in \cref{lem:strong_convexity}. Based on the proof of \cref{lem:strong_convexity}, our strategy is to calculate the minimal eigenvalue of the Hessian matrix.  



First, for $\theta_h = (\theta_{h, 1}, \theta_{h, 2})^\top$, the gradient of $\gL_h (\theta_h)$ is
\begin{align*}
    \nabla \gL_h (\theta_h) &= -\sum_{(s, a) \in \gS \times \gA} \widehat{d^{\expert}_h}(s, a) \sigma (- \langle \phi_h (s,a), \theta_h \rangle) + \sum_{(s, a) \in \gS \times \gA} \widehat{d^{\oU}_h} (s, a)  \sigma \lp  \langle \phi_h (s,a), \theta_h \rangle \rp
    \\
    &= \lp \frac{1}{2} \sigma (\theta_{h, 1}) - \frac{1}{4} \sigma (-\theta_{h, 1}) - \frac{1}{8} \sigma (- \frac{1}{2} \theta_{h, 1} ), \frac{1}{4} \sigma \lp \theta_{h, 2} \rp - \frac{1}{2} \sigma \lp - \theta_{h, 2} \rp - \frac{1}{8} \sigma (- \frac{1}{2} \theta_{h, 2}) \rp^\top.
\end{align*}
Here $\sigma (x) = 1/(1+\exp (-x))$ for $x \in \reals$ is the sigmoid function. Then the Hessian matrix at $\theta_h$ is
\begin{align*}
    \nabla^2 \gL_h (\theta_h) = \begin{pmatrix}
\frac{3}{4} f (\theta_{h, 1}) + \frac{1}{16} f \lp \frac{1}{2} \theta_{h, 1} \rp & 0 \\
0 & \frac{3}{4} f (\theta_{h, 2}) + \frac{1}{16} f \lp \frac{1}{2} \theta_{h, 2} \rp
\end{pmatrix},
\end{align*}
where $f (x) = \sigma (x) (1-\sigma (x))$ and $f(x) = f(-x)$.
For any $t \in [0, 1]$, the eigenvalues of the Hessian matrix at $\theta^t_h = \widebar{\theta}_h + t (\theta^\star_h - \widebar{\theta}_h)$ are
\begin{align*}
\frac{3}{4} f (\theta^t_{h, 1} ) + \frac{1}{16} f \lp \frac{1}{2} \theta^t_{h, 1} \rp, \; \frac{3}{4} f (\theta^t_{h, 2} ) + \frac{1}{16} f \lp \frac{1}{2} \theta^t_{h, 2} \rp. 
\end{align*}
Now, we calculate the minimal eigenvalues of $\nabla^2 \gL_h (\theta^t_h)$. We consider the function 
\begin{align*}
    g(x) = \frac{3}{4} f (x) + \frac{1}{16} f \lp \frac{1}{2} x \rp, \; \forall x \in [a, b]. 
\end{align*}
The gradient is 
\begin{align*}
    g^\prime (x) = \frac{3}{4} \sigma (x) (1-\sigma (x)) (1-2\sigma (x)) + \frac{1}{32} \sigma \lp \frac{1}{2}x \rp \lp 1-\sigma \lp \frac{1}{2}x \rp \rp \lp 1-2\sigma \lp \frac{1}{2}x \rp \rp.  
\end{align*}
We observe that $ \forall x \leq 0, \; g^\prime (x) \geq 0, $ and $\forall x \geq 0, \; g^\prime (x) \leq 0 $. Thus, we have that the minimum of $g (x)$ must be achieved at $x = a$ or $x = b$. Besides, we have that $g (x) = g (-x)$. With the above arguments, we know that the minimal eigenvalue is $g (0.993) \approx 0.163$ and $\tau_h \approx 0.163$.
Then we can calculate that
\begin{align*}
   \sqrt{ \frac{2 \lp \gL_h(\bar{\theta}_h) - \gL_h(\theta^{\star}_h) \rp}{\tau_h}} \approx 0.520,\; \frac{\Delta_h (\bar{\theta}_h)}{L_h} = 1.
\end{align*}
The inequality \eqref{eq:condition} holds.
\end{example}



\subsection{Additional Analysis of WBCU With Function Approximation}
Here we provide an additional theoretical result for WBCU with function approximation when $d = 1$.
\begin{thm}
\label{thm:wbcu_1d}
Consider $d=1$. For any $h \in [H]$, if the following inequality holds
\begin{align}
\label{eq:condition_1d}
    \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \langle \phi_h (s, a), \bar{\theta}_h \rangle < \frac{1}{|\gDE|} \sum_{(s^\prime, a^\prime) \in \gDE_h} \langle \phi_h (s^\prime, a^\prime), \bar{\theta}_h \rangle.
\end{align}
then we have that $\Delta_h (\theta^\star_h) > 0$. Furthermore, the inequality \eqref{eq:condition_1d} is also a necessary condition.
\end{thm}
Theorem \ref{thm:wbcu_1d} provides a clean and sharp condition to guarantee that the learned discriminator can perfectly classify the high-quality samples from $\gDE_h$ and $\gD^{\oS, 1}_h$, and low-quality samples from $\gD^{\oS, 2}_h$. In particular, inequality \eqref{eq:condition_1d} means that by the ground truth parameter $\bar{\theta}_h$, the average score of samples in supplementary dataset is lower than that of samples in expert dataset. This condition is easy to satisfy because the supplementary dataset contains bad samples from $\gD^{\oS, 2}_h$ whose scores are much lower. In contrast, $\gDE$ only contains expert-type samples with high scores.     


\begin{proof}
Recall the objective function
\begin{align*}
    \min_{\theta_h}  \gL_h (\theta_h) = \sum_{(s, a)} \widehat{d^{\expert}_h}(s, a) \log \lp 1 + \exp \lp - \langle \phi_h (s,a), \theta_h \rangle \rp \rp  + \sum_{(s, a)} \widehat{d^{\oU}_h} (s, a)  \log \lp 1 + \exp \lp \langle \phi_h (s,a), \theta_h \rangle \rp \rp.
\end{align*}
Consider the function $f (x) = \log (1+\exp (x))$. We have that $f^{\prime \prime} (x) = \sigmoid (x) (1-\sigmoid (x)) \geq 0$, where $\sigmoid (x) = 1/(1+\exp (-x))$. As such, $f^{\prime \prime} (x)$ is a convex function. Notice that the operations of composition with affine function and non-negative weighted sum preserve convexity \citep{boyd2004convex}. Therefore, $\gL_h (\theta_h)$ is a convex function with respect to $\theta_h$. Then for any $\widetilde{\theta} \in \reals$, it holds that
\begin{align*}
    \gL_h (\theta_h) \geq \gL_h (\widetilde{\theta}) + \nabla \gL_h (\widetilde{\theta}) \lp \theta_h - \widetilde{\theta}  \rp. 
\end{align*}
Setting $\theta_h = \theta^\star_h$ and $\widetilde{\theta} = 0$ yields that 
\begin{align}
\label{eq:convexity_first_order}
    \nabla \gL_h (0) \theta^\star_h \leq \gL_h (\theta^\star_h) - \gL_h (0). 
\end{align}
The gradient of $\gL_h (\theta_h)$ is of the form
\begin{align*}
    \nabla \gL_h (\theta_h) = -\sum_{(s, a) \in \gS \times \gA} \widehat{d^{\expert}_h}(s, a) \sigma (- \langle \phi_h (s,a), \theta_h \rangle) \phi_h (s, a) + \sum_{(s, a) \in \gS \times \gA} \widehat{d^{\oU}_h} (s, a)  \sigma \lp  \langle \phi_h (s,a), \theta_h \rangle \rp \phi_h (s, a).
\end{align*}
Here $\sigmoid (x) = 1/(1+\exp (-x))$ is the sigmoid function. Then we calculate the gradient at $\widetilde{\theta} = 0$.
\begin{align*}
    \nabla \gL_h (0) &= -\sum_{(s, a) \in \gS \times \gA} \widehat{d^{\expert}_h}(s, a) \sigma (0) \phi_h (s, a) + \sum_{(s, a) \in \gS \times \gA} \widehat{d^{\oU}_h} (s, a)  \sigma \lp 0 \rp \phi_h (s, a)
    \\
    &= \frac{1}{2} \lp \frac{\sum_{(s, a) \in \gDU_h} \phi_h (s, a)}{|\gDU|}  - \frac{\sum_{(s, a) \in \gDE_h} \phi_h (s, a)}{|\gDE|}\rp
    \\
    &= \frac{1}{2 |\gDU|} \lp \sum_{(s, a) \in \gDU_h} \phi_h (s, a) - \frac{|\gDU|}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp
    \\
    &= \frac{1}{2 |\gDU|} \lp \sum_{(s, a) \in \gDS_h} \phi_h (s, a) + \sum_{(s, a) \in \gDE_h} \phi_h (s, a) - \frac{|\gDU|}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp
    \\
    &= \frac{1}{2 |\gDU|} \lp \sum_{(s, a) \in \gDS_h} \phi_h (s, a)  - \frac{|\gDS|}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp
    \\
    &= \frac{|\gDS|}{2 |\gDU|} \lp  \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \phi_h (s, a)  - \frac{1}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp. 
\end{align*}
Furthermore, with inequality \eqref{eq:condition_1d}, we know that 
\begin{align*}
    \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \phi_h (s, a)  - \frac{1}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a) \not= 0. 
\end{align*}
Therefore, $\nabla \gL_h (0) \not= 0$. With the first-order optimality condition, we know that $0$ is not the optimal solution and $\gL_h (0) > \gL_h (\theta^\star_h)$. Combined with inequality \eqref{eq:convexity_first_order}, we have that
\begin{align*}
    \nabla \gL_h (0) \theta^\star_h \leq \gL_h (\theta^\star_h) - \gL_h (0) < 0.
\end{align*}
This directly implies that
\begin{align*}
    \lp  \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \phi_h (s, a)  - \frac{1}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp \theta^\star_h < 0.
\end{align*}
Besides, inequality \eqref{eq:condition_1d} implies that
\begin{align*}
    \lp  \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \phi_h (s, a)  - \frac{1}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp \bar{\theta}_h < 0.
\end{align*}
With the above two inequalities, we can derive that $\theta^\star_h \bar{\theta}_h > 0$. Then we have that
\begin{align*}
\Delta_h(\theta^\star_h) &= \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}  \theta^\star_h  \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \theta^\star_h  \phi_h (s^\prime, a^\prime)
\\
     &= \frac{\theta^\star_h}{\bar{\theta}_h} \lp \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}  \bar{\theta}_h  \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \bar{\theta}_h  \phi_h (s^\prime, a^\prime) \rp
     \\
     &=\frac{\theta^\star_h}{\bar{\theta}_h}  \Delta_h(\bar{\theta}_h) 
     \\
     &> 0.
\end{align*}
Thus, the sufficiency of condition \eqref{eq:condition_1d} is proved. Next, we prove the necessity of condition \eqref{eq:condition_1d}. That is, if $\Delta_h (\theta^\star_h) > 0$, then 
\begin{align*}
    \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \langle \phi_h (s, a), \bar{\theta}_h \rangle < \frac{1}{|\gDE|} \sum_{(s^\prime, a^\prime) \in \gDS_h} \langle \phi_h (s^\prime, a^\prime), \bar{\theta}_h \rangle.
\end{align*}
Then we aim to prove that $\theta^\star_h \bar{\theta}_h > 0$. It is easy to obtain that $\theta^\star_h \not= 0$ and $\bar{\theta}_h \not= 0$ since $\Delta_h (\theta^\star_h) > 0$ and $\Delta_h (\bar{\theta}_h) > 0$. Then we consider two cases where $\bar{\theta}_h >0$ and $\bar{\theta}_h <0$.  
\begin{itemize}
    \item Case I ($\bar{\theta}_h >0$). In this case, we have that
    \begin{align*}
        \Delta_h (\bar{\theta}_h) &= \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}  \bar{\theta}_h  \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \bar{\theta}_h  \phi_h (s^\prime, a^\prime)
        \\
        &= \bar{\theta}_h \lp \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime)  \rp.
    \end{align*}
    Then $\Delta_h (\bar{\theta}_h) > 0$ implies that
    \begin{align}
    \label{eq:min>max}
        \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) > \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime).
    \end{align}
    Then we claim that $\theta^\star_h > 0$. Otherwise, it holds that
    \begin{align*}
         \Delta_h (\theta^\star_h) &= \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}  \theta^\star_h \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \theta^\star_h  \phi_h (s^\prime, a^\prime)
        \\
        &= \theta^\star_h \lp \max_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) - \min_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime)  \rp
        \\
        &< 0.
    \end{align*}
    The last inequality follows $\theta^\star_h < 0$ and $\max_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) - \min_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime) > 0$ due to inequality \eqref{eq:min>max}. Thus, the above inequality conflicts with $\Delta_h (\theta^\star_h) > 0$. The claim that $\theta^\star_h > 0$ is proved and $\bar{\theta}_h \theta^\star_h > 0$.
    \item Case II ($\bar{\theta}_h < 0$). Similarly, we get that 
    \begin{align*}
        \Delta_h (\bar{\theta}_h) &= \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}  \bar{\theta}_h  \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \bar{\theta}_h  \phi_h (s^\prime, a^\prime)
        \\
        &= \bar{\theta}_h \lp \max_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) - \min_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime)  \rp.
    \end{align*}
    Then $\Delta_h (\bar{\theta}_h) > 0$ implies that
    \begin{align}
    \label{eq:max<min}
        \max_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) < \min_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime).
    \end{align}
    Similar to the analysis in case I, we claim that $\theta^\star_h < 0$. Otherwise, it holds that
    \begin{align*}
         \Delta_h (\theta^\star_h) &= \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h}  \theta^\star_h \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \theta^\star_h  \phi_h (s^\prime, a^\prime)
        \\
        &= \theta^\star_h \lp \min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime)  \rp
        \\
        &< 0.
    \end{align*}
    The last inequality follows $\theta^\star_h > 0$ and $\min_{(s, a) \in \gDE_h \cup \gD^{\oS, 1}_h} \phi_h (s, a) - \max_{(s^\prime, a^\prime) \in \gD^{\oS, 2}_h}  \phi_h (s^\prime, a^\prime) < 0$ due to inequality \eqref{eq:max<min}. Thus, the above inequality conflicts with $\Delta_h (\theta^\star_h) > 0$. The claim that $\theta^\star_h < 0$ is proved and $\bar{\theta}_h \theta^\star_h > 0$.
\end{itemize}
To summarize, we have proved that $\bar{\theta}_h \theta^\star_h > 0$. Similar to the proof of the sufficient condition, by the convexity of $\gL_h (\theta_h)$ and optimality of $\theta^\star_h$, we can obtain that
\begin{align*}
    \lp  \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \phi_h (s, a)  - \frac{1}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp \theta^\star_h < 0.
\end{align*}
This directly implies that
\begin{align*}
    \lp  \frac{1}{|\gDS|} \sum_{(s, a) \in \gDS_h} \phi_h (s, a)  - \frac{1}{|\gDE|}  \sum_{(s, a) \in \gDE_h} \phi_h (s, a)   \rp \bar{\theta}_h < 0,
\end{align*}
which completes the proof of necessity.

\end{proof}
